First Measurement of the Ratio of Branching Fractions B(Lambda_b to Lambda_c mu nu)/B(Lambda_b to Lambda_c pi)

The analysis uses data from an integrated luminosity of approximately 172 pb-1 of ppbar collisions at sqrt(s)=1.96 TeV, collected with the CDF II detector at the Fermilab Tevatron. The Lambda_b and B0 relative branching fractions are measured to be: B(Lambda_b to Lambda_c+ mu nu)/B(Lambda_b to Lambda_c+ pi) = 16.6 +- 3.0 (stat) +- 1.0 (syst) +2.6 -3.4 (PDG) +- 0.3 (EBR), B(B0 to D+ mu nu)/B(B0 to D+ pi) = 9.9 +- 1.0 (stat) +- 0.6 (syst) +- 0.4 (PDG) +- 0.5 (EBR), B(B0 to D*+ mu nu)/B(B0 to D*+ pi) = 16.5 +- 2.3 (stat) +- 0.6 (syst) +- 0.5 (PDG) +- 0.8 (EBR) This article also presents measurements of the branching fractions of four new Lambda_b semileptonic decays: Lambda_b to Lambda_c(2595)+ mu nu, Lambda_b to Lambda_c(2625)+ mu nu, Lambda_b to Sigma_c(2455)0 pi mu nu, Lambda_b to Sigma_c(2455)++ pi mu nu, relative to the branching fraction of the Lambda_b to Lambda_c mu nu decay. Finally, the transverse-momentum distribution of Lambda_b baryons produced in p-pbar collisions is measured and found to be significantly different from that of B0 mesons.

==> response_20081208 <==
Dear PRD Referees,

We thank the referees for their reports. Our responses to the individual 
comments and a summary of the changes made are below. 

-------------------------------------------------------------------------
Report of Referee A:
-------------------------------------------------------------------------

p.10, eq.1: not all variables are introduced (although obvious), namely
N_inclsemi and N_semibg

Ans: We introduced the variables "N_inclsemi" and "N_semibg" after eq.1 
        when we described our analysis procedure. As the referee pointed out, 
        the definitions of these two variables were obvious. We chose not to 
	modify our text.


p.12, l.6: use opposite-charge instead of opposite-sign (jargon)? 

Ans: Changed to "oppositely-charged".

p.13, l.14: bg reduction 50%, signal 90% eff. - you know that from
Monte Carlo?

Ans: The relativistic kinematics of Lambda_b predicts that protons have higher 
	pt on average. We confirmed this with Monte Carlo. We used 
	Monte Carlo to estimate the signal efficiency and sideband 
	data to estimate the background reduction. 

p.16, l. 3: BGENERATOR - no reference given

Ans: The BGENERATOR is a CDF internal program. Unfortunately, it does 
	not have a documentation accessible to the public. 
	We added a footnote in the paper to briefly define B generator. 

p.16, last lines, p.17 first lines, also fig. 4: the term 'scaling'
might be misleading as in my eyes scaling implies a common factor for
all bins. I would prefer an expression like 'bin-by-bin correction'

Ans: We changed the term "scaling" to "multiplied", and 
"scaled distribution" to "corrected distribution".


p.30, section B, heading: \sigma_B^0 - the bar above B^0 seems to be
missing, also on the same page in the definitions of G, rho. Same issue
with: ratios p.35 l.3, p.44 eq.A3, p.46 eq.C2, maybe elsewhere

Ans: We modified all B^0 in our text and figures to \bar{B}^0.

p.54, fig.1: 'I' marks the displaced vertex in the sketch?

Ans: Yes, that's correct. Since 'I' was not needed, we 
     removed the label.

p. 58, fig. 6: even though a reference is given, what is the reason for
negative probabilities - background subtraction?

Ans: Yes, it is because of background subtraction. 

-------------------------------------------------------------------------
Report of Referee B:
-------------------------------------------------------------------------

This paper provides a measurement of the relative branching fractions of
the lambda_b baryon to the simplest of the pure hadronic and semileptonic
final states.  Branching fractions of the lambda_b have not been studied
very extensively, and the new information from this measurement is useful.
The analysis has been done with care and is well described in the paper.
I support its publication in Phys. Rev. D.

Most of the few questions that arose in my reading were answered in the
text.  Some comments for the authors to consider:

Fig. 1 caption:  I suggest adding a phrase:  "the d0" -> "the
d0 of each pion", or "the d0's of both pions".  I was puzzled at
first that the caption meant that only the d0 given as illustration satisfied
the trigger.

Ans: We modified the caption to clarify this. 

p. 14, paragraph preceding the one containing Eqs. 2,3, 5th and 6th lines
from the bottom:  The mass ranges of the selection are given.  I suggest
adding a forward reference to Fig.2 so that the reader appreciates why
these numbers are appropriate.

Ans: Added "(see Fig. 2)".

Fig. 8 caption:  The sentence "Note that the backgrounds are concentrated
in the low mass region." seems too strong a statement given the curves.
The curves seem to show that the signal to background is only somewhat
improved by the cut, even allowing for the distortion caused by the
log scale.


Ans: We softened our sentence and removed the term "concentrated".

p. 26, first para of sect. VII, last two lines:  I didn't understand the
point that the ratio of estimated BF's need not be the same as the final
measured result.  Ideally you would iterate after finding the result,
or is it being claimed that in this context a different ratio would
be appropriate?

Ans: Our result need not be the same as the input ratio since the
     input ratio is used to estimate backgrounds from b hadron decays
     in the inclusive semileptonic sample (N_feed term in eqn 6).
     These backgrounds amount to approximately 24% of the inclusive
     semileptonic sample (Table V).
     We chose a direct calculation of the ratio rather than an
     iterative approach to avoid complexity in obtaining and propagating
     uncertainties.


p. 20, last para of sect. V A, the use of the term "b meson" should
be defined (assuming I didn't miss such a definition earlier), since it's
not a standard notation (b and c are quarks, not mesons).  Since this and
"c meson" are used further, the intent becomes fairly obvious, but
looks
like a mistake on the first encounter. 

Ans: We added a definition when we used "b meson" the first time when it 
     appeared in this paper (Section 1). The definition of "c meson" follows 
     the same definition.

I noticed an occasional run-on sentence, such as p. 19, next-to-last
sentence before the start of sect. V A:  "simulation and the parameter
values are obtained" -> "simulation with parameter values that are
obtained".

Ans: We broke up the long sentence and made it easier to read now.


----------------------------------------------------------------------------
                         
                          Summary of the change made 
----------------------------------------------------------------------------

Figures:

1 : Remove the symbol "I" from the figure and clarified the d0 and Lxy in 
   the caption

3b: B^0 --> \bar{B}^0 in the title of x axis

4b: FF-scaled --> FF-corrected in the legend. 
    Replaced "scaling" with "corrected" in the caption. 

8: Changed the caption. Replaced the term "concentrated".

10: B^0 --> \bar{B}^0 in the title of y axis of lower plot

11b and d: B^0 --> \bar{B}^0 in the title of y axis

16: The figure was produced in PAW. Changed to ROOT format, so that the 
    background is not black in the pdf file.

----------------------------------------------------------------------------
Text: 

General: Changed all B^0 to \bar{B}^0.

Detailed: 

Section 1:
Added definition of $b$ meson

Section 2: 
opposite-sign--> oppositely-charged

Section 3:
Added a forward reference to Fig 2 when mentioning the mass window cuts

Section 4A:
Added a reference to Bgenerator 

        4C:
Replaced the term "scaling" with "multiplied", and "scaled distribution" to "corrected distribution".

Section 5A:

Break the long sentence "The functional form for each combined background 
spectrum is determined empirically to match the shape of simulated 
mass distribution and the parameter values are obtained by fitting the 
simulated spectrum.".



